A Robot by Any Other Frame: Framing and Behaviour Influence Mind Perception in Virtual but not Real-World Environments

Mind perception in robots has been an understudied construct in human-robot interaction (HRI) compared to similar concepts such as anthropomorphism and the intentional stance. In a series of three experiments, we identify two factors that could potentially influence mind perception and moral concern in robots: how the robot is introduced (framing), and how the robot acts (social behaviour). In the first two online experiments, we show that both framing and behaviour independently influence participants' mind perception. However, when we combined both variables in the following real-world experiment, these effects failed to replicate. We hence identify a third factor post-hoc: the online versus real-world nature of the interactions. After analysing potential confounds, we tentatively suggest that mind perception is harder to influence in real-world experiments, as manipulations are harder to isolate compared to virtual experiments, which only provide a slice of the interaction.

==> HRI2020 Tower of Hanoi Paper/experiment3-table.tex <==
\begin{table}
\caption{Results Experiment 3}
\label{tab:experiment3-means}
\begin{tabular}{@{}p{0.15\linewidth}lllllll@{}}
\toprule
               & behavior   & framing     & Mean    & SD  & N & M & F \\

\midrule
\multirow{2}{0.15\linewidth}{Mind Perception} & non-social & low-mind & 2.15 & .89 & 25 &17&8                  \\
               &            & high-mind & 2.48 & .64 & 24 &16&8                   \\
               &            & total       & 2.31 & .79 & 49 &33&16                   \\\cmidrule{2-8}
               & social     & low-mind & 2.47 & .86 & 25  &14&11                  \\
               &            & high-mind & 2.54 & .73 & 25 &14&11                   \\
               &            & total       & 2.50 & .79 & 50 &28&22                   \\\cmidrule{2-8}
               & total      & low-mind & 2.31 & .88 & 50  &31&19                  \\
               &            & high-mind & 2.50 & .68 & 49 &30&19                   \\
               &            & total       & 2.40 & .79 & 99 &61&38                   \\\midrule
\multirow{2}{0.15\linewidth}{Moral Concern}   & non-social & low-mind & 5.17 & .84 & 25  &17&8\\
               &            & high-mind & 5.18 & .79 & 24 &16&8                   \\
               &            & total       & 5.17 & .81 & 49 &33&16                   \\\cmidrule{2-8}
               & social     & low-mind & 5.07 & .84 & 25  &14&11                  \\
               &            & high-mind & 5.09 & .56 & 25 &14&11                   \\
               &            & total       & 5.08 & .60 & 50 &28&22                   \\\cmidrule{2-8}
               & total      & low-mind & 5.12 & .74 & 49  &31&19                  \\
               &            & high-mind & 5.13 & .68 & 50 &30&19                   \\
               &            & total       & 5.13 & .71 & 99 &61&38                   \\\midrule
Godspeed       & non-social & low-mind & 3.53 & .85 & 25  &17&8                  \\
               &            & high-mind & 3.8  & .57 & 24 &16&8                   \\
               &            & total       & 3.67 & .73 & 49 &33&16                   \\\cmidrule{2-8}
               & social     & low-mind & 3.63 & .61 & 25  &14&11                  \\
               &            & high-mind & 3.6  & .56 & 25 &14&11                   \\
               &            & total       & 3.61 & .58 & 50 &28&22                   \\\cmidrule{2-8}
               & total      & low-mind & 3.58 & .73 & 49  &31&19                  \\
               &            & high-mind & 3.70 & .57 & 50 &30&19                   \\
               &            & total       & 3.64 & .66 & 99 &61&38                  \\\bottomrule
\end{tabular}
\end{table}
